Towards Attention-based Contrastive Learning for Audio Spoof Detection

Vision transformers (ViT) have made substantial progress for classification tasks in computer vision. Recently, Gong et. al. '21, introduced attention-based modeling for several audio tasks. However, relatively unexplored is the use of a ViT for audio spoof detection task. We bridge this gap and introduce ViTs for this task. A vanilla baseline built on fine-tuning the SSAST (Gong et. al. '22) audio ViT model achieves sub-optimal equal error rates (EERs). To improve performance, we propose a novel attention-based contrastive learning framework (SSAST-CL) that uses cross-attention to aid the representation learning. Experiments show that our framework successfully disentangles the bonafide and spoof classes and helps learn better classifiers for the task. With appropriate data augmentations policy, a model trained on our framework achieves competitive performance on the ASVSpoof 2021 challenge. We provide comparisons and ablation studies to justify our claim.

==> 06.ablation.tex <==
\section{Ablation}
\label{sec:ablation}

\subsection{Limitations and future work}
The following avenues could further improve model performance:
    \begin{enumerate}
    \item Contrastive mix-up could speed up training convergence and possibly impprove model performance 
    \item Sampling strategy where {\em hard to learn} samples (e.g. VC-type samples) are given more importance
        \item A grid search over the hyperparameters in the proposed model: optimizer, learning rates, and batch size could potentially improve the reported performance.
        \item Similarity measures other than cosine similarity, e.g. \cite{saeed2021contrastive}
    \end{enumerate}

Discussion on comparison with wav2vec2.0-based models:
\noindent\textbf{Comparison with Wav2vec2.0 model \cite{tak2022automatic}}
\begin{enumerate}
        \item Wav2vec2.0 is a bigger model with $317$ million parameters, as opposed to $5.73$ million parameters in our ViT model;
        \item Pre-trained on a big multi-lingual only-speech dataset ; We train on AudioSet, where there are 1 million speech samples; 
\end{enumerate}
